Technical Report: Beaconless Geo-Routing Under The Spotlight: Practical Link Models and Application Scenarios

Analysis and simulation of beaconless geo-routing protocols have been traditionally conducted assuming equal communication ranges for the data and control packets. In reality, this is not true since the communication range is actually function of the packet length. Control packets are typically much shorter than data packets. As a consequence, a substantial discrepancy exists in practice between their respective communication ranges. In this paper, we devise a practical link model for computing the effective communication range. We further introduce two simple strategies for bridging the gap between the control and data packet communication ranges. Our primary objective in this paper is to construct a realistic analytical framework describing the end-to-end performance of beaconless geo-routing protocols. Two flagship protocols are selected in this paper for further investigation under the developed framework. For a better perspective, the two protocols are actually compared to a hypothetical limit case; one which offers optimal energy and latency performance. Finally, we present four different application scenarios. For each scenario, we highlight the geo-routing protocol which performs the best and discuss the reasons behind it.

==> IEEEtran5/README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> README <==
Manifest and Documentation for the `subfig' package (version 1.3).
------------------------------------------------------------------------

This directory contains version 1.3 of the subfig package.  In a UNIX
or UNIX-like command shell, use `make' to extract the subfig package
and run the local tests.


MANIFEST:
---------
  The following files as well as the derivative files `subfig.sty' and
  `altsf.cfg' constitute the subfig package and are considered as "the
  work" under the LaTeX Project Public License (LPPL 1.3 or later).

Makefile           UNIX makefile to extract the subfig package
                       and related material.
README             This file.
subfig.dtx         The documented subfig package.
subfig.ins         The subfig package installation file.
subfig.pdf         The subfig package documentation (in PDF).
test1.tex          Test one: Basic checks and examples.
test2.tex          Test two: Check for extra space around figure
test3.tex          Test four: Test of optional args and \subref.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test of continued figures.
test6.tex          Test six: Test of options and option interaction.
test7.tex          Test seven: Test of class/package misuse of \let.


FILES AFTER `make':
-------------------
Makefile           UNIX makefile to extract the subfig package
                       and related material.
README             This file.
altsf.cfg          A subfig configuration file (which make the subfig 
                        package act similar to the subfigure package).
ltxdoc.cfg         Configuration file to print change history and
                       index on the subfig package documentation.       
subfig.dtx         The documented subfig package.
subfig.ins         The subfig package installation file.
subfig.pdf         The subfig package documentation (in PDF).
subfig.ps          The subfig package documentation (in PostScript).
subfig.sty         The subfig package 
test1.ps           Results of test one.
test1.tex          Test one: Basic checks and examples.
test2.ps           Results of test two.
test2.tex          Test two: Check for extra space around figure
test3.ps           Results of test three.
test3.tex          Test four: Test of optional args and \subref.
test4.pdf          Results of test four.
test4.tex          Test four: Test of interaction with hyperref.
test5.ps           Results of test five.
test5.tex          Test five: Test of continued figures.
test6.ps           Results of test six.
test6.tex          Test six: Test of options and option interaction.
test7.tex          Test seven: Test of class/package misuse of \let.
test7a.ps          Log from test seven run.
test7b.ps          Results of test seven.


NOTES:
------

1. To verify the results of the test(s) (which are run using the
   preferred options), compare with the test(s) found at:
   http://www.cs.cmu.edu/~sdc/latex/subfig.13/

2. This version of the subfig package removes a "feature" which
   allowed a line break to occur between two subfloats separated
   by whitespace instead of requiring an explicit "\\".  If this
   "feature" was used to position sub-floats, they may now be
   incorrectly displayed.

   If this occurs, the solution is to add an expicit linebreak
   between the problem sub-floats.  For example, the following
   to the left would seem to work correctly, but suppressed
   the "farskip" placing the figures too close together and 
   will, now, no longer work.  It should be written as on the
   left.

   \begin{figure}                  \begin{figure}		
     \centering	                     \centering		
       \subfloat[One.]{...}%	       \subfloat[One.]{...}	
     \hspace{.25in}%		     \hspace{.25in}%		
       \subfloat[Two.]{...}	       \subfloat[Two.]{...} \\	
       \subfloat[Three.]{...}%         \subfloat[Three.]{...}	
     \hspace{.25in}%		     \hspace{.25in}%		
       \subfloat[Four.]{...}%	       \subfloat[Four.]{...}	
     \caption{Simple Case.}	     \caption{Simple Case.}	
   \end{figure}                    \end{figure}               










